Listenability of Synthetic Speech: On the Effect of Linguistic Registers in Text-to-Speech Input

With the rapid advancement of Large Language Models (LLMs), LLM-generated text is increasingly being used as input for speech synthesis, yet little is known about its listenability compared to other linguistic registers. This paper presents a preliminary study of listenability across conversational, formal written, simplified written, and LLM-generated registers in terms of listener effort and comprehension during synthesized delivery. An experiment with 47 participants measured subjective mental effort, cognitive load, and cued recall in a within subjects design. Register characteristics were examined through readability metrics and Biber's Multi-Dimensional Analysis. Our findings indicate higher listenability for synthesized speech from written sources compared to radio transcripts, demonstrating the intricacies of language and register. Furthermore, LLM-generated text was as listenable as Wikipedia-sourced text, supporting its suitability in synthetic speech applications.

==> rebuttal.tex <==
We thank the reviewers for their constructive feedback. We address the most substantive points below. 

Reviewer 2: The conditions compared do not share semantic contents. 
We acknowledge that the four conditions vary in semantic content alongside register, and will expand the limitations section accordingly. Two considerations mitigate the concern: First, the ART effect is consistent across four topically diverse samples, whereas a content-driven explanation would predict greater variability. Second, the design prioritises ecological validity, as real TTS pipelines ingest naturally-occurring text in which register and content co-vary. Paraphrasing across registers to hold semantic content constant is a valuable direction for follow-up work, which we will flag in the revision. 

Reviewer 3: Limited novelty contribution. 
Reviewer 3 identifies the work as addressing "the critical gap regarding whether LLM-generated text is suitable as input for Text-to-Speech systems" and describes this as a "Novel Research Question." The novelty score, however, cites prior work establishing that register affects readability and listening. Our contribution is not that register varies, which is well established, but the TTS-specific empirical finding that conversational transcripts produce the least listenable synthesised speech, and that LLM-generated text is statistically indistinguishable from curated written sources on listenability measures. We will sharpen the framing of contributions in Section 1 accordingly. 

Reviewer 3: Technical correctness. 
The weaknesses paragraph in R3 raises concerns regarding novelty but identifies no specific methodological issue. We welcome guidance from the meta-reviewer on any technical point we should address. 

Reviewer 2: Minor clarifications. 
ART comprises multi-party talkback radio (host and callers). The camera-ready paper will note this, add word count and dependency depth for ART in Table 2, and include example AIME and NASA TLX items.

We thank the reviewers and meta-reviewer for their consideration.

Rv1: "Have a Future Work section"
Section 5.3 Limitations and future directions serves this purpose. Will be extended in the final version to outline the next steps and guidance on how the research can be developed.

RV2: "The conditions compared do not share semantic contents".
We agree with this comment. 
We describe in Section 3.3 the efforts we have made to ensure an overlap of semantic contents between the stimuli, including matching the topics/themes across conditions. 
The revision will include a discussion of how semantic content differences could be a confounding factor.

Rv2: "ART should definitely be included in Table 2".
We decided to exclude...
The revised table will include ART and the metrics that are valid for transcripts () to provide relevant context.

Rv3: "limited novelty".


